Multi-resolution Monocular Depth Map Fusion by Self-supervised Gradient-based Composition

Monocular depth estimation is a challenging problem on which deep neural networks have demonstrated great potential. However, depth maps predicted by existing deep models usually lack fine-grained details due to the convolution operations and the down-samplings in networks. We find that increasing input resolution is helpful to preserve more local details while the estimation at low resolution is more accurate globally. Therefore, we propose a novel depth map fusion module to combine the advantages of estimations with multi-resolution inputs. Instead of merging the low- and high-resolution estimations equally, we adopt the core idea of Poisson fusion, trying to implant the gradient domain of high-resolution depth into the low-resolution depth. While classic Poisson fusion requires a fusion mask as supervision, we propose a self-supervised framework based on guided image filtering. We demonstrate that this gradient-based composition performs much better at noisy immunity, compared with the state-of-the-art depth map fusion method. Our lightweight depth fusion is one-shot and runs in real-time, making our method 80X faster than a state-of-the-art depth fusion method. Quantitative evaluations demonstrate that the proposed method can be integrated into many fully convolutional monocular depth estimation backbones with a significant performance boost, leading to state-of-the-art results of detail enhancement on depth maps.

==> exp_old.tex <==

\section{Experiments}\label{sec:experiments}

In this section, we firstly introduce the benchmark datasets used in evaluations in Section~\ref{sec:dataset}. We compare the proposed method with several state-of-the-art monocular depth estimation methods and depth refinment methods in Section~\ref{sec:comparison}, where our method outperforms both quantitatively and qualitatively. Lastly, We conduct several ablations to study the effectiveness of several special design in our pipeline in Section~\ref{sec:ablations}. More comparisons, ablations can be found in the supplement. 

% \begin{table*}[t]
% 	\centering 
% 	\scalebox{0.7}{
% 		\begin{tabular}{c| c| c c c| c c c| c c c| c c c|c} 
% 			\hline 
% 			\multirow{2}{*}{Methods}&\multicolumn{3}{c|}{KITTI (1216*352)}&\multicolumn{3}{c|}{NYU (640*480)}&\multicolumn{3}{c|}{Sinten (1024*436)}&\multicolumn{3}{c|}{Diode (1024*768)}&	\multirow{2}{*}{Rank}\\
% 			&&AbsRel$\downarrow$&log$10\downarrow$&$\delta_{1.25}\uparrow$&AbsRel$\downarrow$&log$10\downarrow$&$\delta_{1.25}\uparrow$&AbsRel$\downarrow$&log$10\downarrow$&$\delta_{1.25}\uparrow$&AbsRel$\downarrow$&log$10\downarrow$&$\delta_{1.25}\uparrow$&\\
% 		\hline	
% 		SGR~\cite{xian2020structure}&0.419&0.158&0.39&0.168&0.063&0.773&0.85&0.225&0.362&0.479&0.107&0.592&6.50\\
% 		MiDaS~\cite{ranftl2019towards}&0.422&0.156&0.392&0.159&0.053&0.801&0.856&0.224&0.359&0.458&0.092&0.612&5.83\\
% 		DiverseDepth~\cite{yin2020diversedepth}&0.378&0.147&0.422&0.131&0.052&0.844&0.87&0.23&0.362&0.39&\bf{0.085}&0.663&5.00\\
		
% 		LeRes~\cite{yin2021learning}&0.191&0.081&0.681&\bf{0.093}&\bf{0.039}&\bf{0.907}&0.48&\underline{0.108}&0.556&\underline{0.354}&\underline{0.086}&\bf{0.7}&2.33\\
		
% 		LeRes~\cite{yin2021learning}&0.189&0.082&0.677&0.112&0.046&0.878&\underline{0.448}&\bf{0.104}&\underline{0.562}&0.361&0.092&0.681&3.08\\
		
% 		\hline
% 		Ours&\underline{0.179}&\underline{0.077}&\underline{0.701}&\underline{0.105}&\underline{0.044}&\underline{0.889}&0.446&0.116&\bf{0.563}&\underline{0.354}&0.092&\bf{0.7}&2.08\\
% 		Ours&\bf{0.165}&\bf{0.07}&\bf{0.742}&0.118&0.049&0.868&\bf{0.438}&0.115&0.56&\bf{0.352}&0.099&0.682&2.66\\
		
% 			\hline
% 		\end{tabular}
% 	}
% 	\caption{The quantitative evaluations on four benchmark datasets. Ours with the ResNet50 encoder parameters is the best one among all methods. Ours with the ResNeXt101 encoder is the third place among all methods. }\label{table:quantitative} 
% \end{table*}


\begin{table*}
\centering
\scalebox{0.85}{
\begin{tabular}{c|c|ccccccc|ccccccc} 
\hline
\multirow{2}{*}{Type} & \multirow{2}{*}{Methods} & \multicolumn{7}{c|}{Multiscopic} & \multicolumn{7}{c}{Middlebury2021} \\ 
\cline{3-16}
 &  & AbsRel\downarrow & SqRel\downarrow & rms\downarrow & log10\downarrow & \delta_{1}\uparrow & \delta_{2}\uparrow & \delta_{3}\uparrow & AbsRel\downarrow & SqRel\downarrow & rms\downarrow & log10\downarrow & \delta_{1}\uparrow & \delta_{2}\uparrow & \delta_{3}\uparrow \\ 
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Monocular\\Estimation\end{tabular}} & SGR & \uline{0.314} & 0.081 & 0.120 & 0.086 & 0.745 & 0.904 & \textbf{0.949} & 0.181 & 0.028 & 0.103 & 0.072 & 0.758 & 0.927 & 0.978 \\
 & LeRes & 0.320 & 0.079 & 0.111 & \uline{0.082} & \uline{0.776} & 0.909 & 0.948 & \textbf{0.143} & \textbf{0.021} & \uline{0.089} & \textbf{0.056} & 0.834 & \textbf{0.955} & \uline{0.983} \\ 
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Guided\\Filter\end{tabular}} & SGR-GF & 0.318 & 0.082 & 0.121 & 0.087 & 0.743 & 0.903 & 0.948 & 0.180 & 0.028 & 0.102 & 0.071 & 0.758 & 0.927 & 0.978 \\
 & LeRes-GF & 0.317 & \uline{0.078} & \uline{0.110} & \uline{0.082} & \uline{0.776} & \uline{0.910} & \textbf{0.949} & \textbf{0.143} & \textbf{0.021} & 0.089 & \textbf{0.056} & \uline{0.834} & \uline{0.954} & \uline{0.983} \\ 
\hline
\multicolumn{1}{l|}{\multirow{2}{*}{Depth refinement}} & 3DK & 0.366 & 0.098 & 0.129 & 0.094 & 0.730 & 0.895 & 0.940 & 0.166 & 0.023 & 0.101 & 0.068 & 0.745 & 0.945 & \textbf{0.993} \\
\multicolumn{1}{l|}{} & BMD & 0.323 & 0.079 & \uline{0.110} & \uline{0.082} & 0.773 & \uline{0.910} & \textbf{0.949} & 0.150 & 0.023 & 0.091 & 0.059 & 0.829 & 0.946 & 0.979 \\ 
\hline
\multirow{2}{*}{Ours} & SGR-Ours & 0.318 & 0.082 & 0.122 & 0.088 & 0.742 & 0.902 & 0.948 & 0.180 & 0.027 & 0.101 & 0.072 & 0.761 & 0.925 & 0.977 \\
 & LeRes-Ours & \textbf{0.307} & \textbf{0.072} & \textbf{0.109} & \textbf{0.081} & \textbf{0.781} & \textbf{0.912} & \textbf{0.949} & \textbf{0.143} & \textbf{0.021} & \textbf{0.087} & \uline{0.057} & \textbf{0.835} & 0.953 & \uline{0.983} \\
\hline
\end{tabular}}
\end{table*}

\begin{table*}
\centering
\scalebox{0.85}{
\begin{tabular}{c|c|ccccccc|ccccccc} 
\hline
\multirow{2}{*}{Type} & \multirow{2}{*}{Methods} & \multicolumn{7}{c|}{Hypersim} & \multicolumn{7}{c}{Diodo} \\ 
\cline{3-16}
 &  & AbsRel\downarrow & SqRel\downarrow & rms\downarrow & log10\downarrow & \delta_{1}\uparrow & \delta_{2}\uparrow & \delta_{3}\uparrow & AbsRel\downarrow & SqRel\downarrow & rms\downarrow & log10\downarrow & \delta_{1}\uparrow & \delta_{2}\uparrow & \delta_{3}\uparrow \\ 
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Monocular\\Estimation\end{tabular}} & SGR & 0.421 & 3.885 & 6.713 & 0.155 & 0.446 & 0.707 & 0.859 & 0.132 & 0.035 & 0.051 & 0.034 & 0.934 & 0.975 & \uline{0.987} \\
 & LeRes & 0.288 & 2.252 & 5.543 & 0.118 & \uline{0.604} & 0.805 & \uline{0.913} & \uline{0.074} & 0.016 & \textbf{0.037} & \textbf{0.021} & \textbf{0.965} & \uline{0.989} & \textbf{0.994} \\ 
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Guided\\Filter\end{tabular}} & SGR-GF & 0.422 & 3.810 & 6.646 & 0.155 & 0.445 & 0.706 & 0.861 & 0.132 & 0.035 & \uline{0.050} & 0.034 & 0.934 & 0.975 & \uline{0.987} \\
 & LeRes-GF & 0.293 & 2.293 & 5.576 & 0.119 & 0.600 & 0.802 & 0.912 & \textbf{0.073} & \uline{0.015} & \textbf{0.037} & \textbf{0.021} & \uline{0.964} & \uline{0.989} & \textbf{0.994} \\ 
\hline
\multicolumn{1}{l|}{\multirow{2}{*}{Depth  refinement}} & 3DK & 0.477 & 4.573 & 6.182 & 0.158 & 0.486 & 0.719 & 0.892 & 0.746 & 0.207 & 0.155 & 0.226 & 0.42 & 0.617 & 0.736 \\
\multicolumn{1}{l|}{} & BMD & \textbf{0.280} & \textbf{2.086} & \uline{5.399} & \uline{0.117} & 0.601 & \textbf{0.814} & 0.879 & 0.080 & 0.019 & 0.077 & 0.039 & 0.903 & 0.967 & 0.984 \\ 
\hline
\multirow{2}{*}{Ours} & SGR-Ours & 0.414 & 3.583 & 6.357 & 0.152 & 0.457 & 0.711 & 0.861 & 0.131 & 0.034 & \uline{0.050} & 0.034 & 0.933 & 0.975 & 0.986 \\
 & LeRes-Ours & \uline{0.285} & \uline{2.109} & \textbf{5.355} & \textbf{0.115} & \textbf{0.605} & \uline{0.813} & \textbf{0.924} & \textbf{0.073} & \textbf{0.014} & \textbf{0.037} & \uline{0.022} & \textbf{0.965} & \textbf{0.990} & \textbf{0.994} \\
\hline
\end{tabular}}
\caption{The quantitative evaluations on two benchmark datasets. Bold numbers denote the best result while underlined numbers are second best.}\label{table:quantitative}
%\vspace{-20pt}
\end{table*}

%\subsection{Training details}\label{sec:details}
 %\red{More intermediate results such as visualizations of activation at each layer are included in the supplementary material. }

\subsection{Benchmark datasets and evaluation metrics}\label{sec:dataset}
To evaluate the depth estimation ability of our method, we adopt four zero-shot datasets, which are Multiscopic~\cite{yuan2021stereo},  Middlebury~\cite{scharstein2014high}, Hypersim~\cite{roberts:2021} and Diode~\cite{vasiljevic2019dode}. All benchmark datasets are unseen during training. 

Multiscopic~\cite{yuan2021stereo} dataset is an indoor dataset including real data collected by multi-eye cameras and synthetic data rendered by 3D engines. The dataset contains 1100 scenes of synthetic data for training, 100 scenes of synthetic data for testing and 100 scenes of real data for other tasks. For each synthetic scene, Multiscopic~\cite{yuan2021stereo} provide 5 different views of rgb image and disparity, at a resolution of $1280x1080$. And for each real scene, it provide 3 different views of rgb image and disparity.


Middlebury2021~\cite{scharstein2014high} is a high quality stereo dataset collected by a structured light acquisition system. This dataset provides images and disparities for different indoor scenes at a resolution of $1920\times1080$. The dataset contains 24 testing scenes with their calibration files respectively. At test time, we change the floating-point disparity value $d$ to depth value $z$ by $z = baseline * f / (d + d_{offs})$, where the values of  $baseline$, the focal length $f$ and the displacement of principal points $d_{offs}$ are provided in the dataset.

Hypersim~\cite{roberts:2021} is a photorealistic synthetic dataset for holistic indoor scene understanding. It contains 77400 images of 461 indoor scenes with per-pixel labels and corresponding ground truth geometry. Due to the large size of the whole dataset, we test on three subsets containing 286 tone-mapped images generated from their released code.

Diode (Dense Indoor and Outdoor DEpth)~\cite{vasiljevic2019dode} is a dataset of high-resolution RGB-D images of various indoor and outdoor scenes. 

%In our evaluations, for NYU dataset we test on the testing set of 654 images. For KITTI dataset, the released validation dataset of 1000 images are used for evaluation. For DIODE, we use their validation dataset of 771 images including both indoor and outdoor data. For Sintel dataset, we sample 15 sequences containing 740 images. For Ibims-1, we test on the whole dataset of 100 images. 

In our evaluations, we test on the whole Middlebury2021~\cite{scharstein2014high}, including 24 real scenes. For Multiscopic~\cite{yuan2021stereo} dataset, we evaluate on synthetic test data, containing 100 high resolution indoor scenes. For Hypersim~\cite{roberts:2021}, we evaluate on three subsets of 286 tone-mapped images generated by the released codes. For Diode~\cite{vasiljevic2019dode}, we use their validation dataset of 771 images including both indoor and outdoor data. On these datasets, we evaluate several error metrics as follows: The absolute relative error $AbsRel$ is defined as: $AbsRel=\frac{1}{N}\sum\left\|\frac{d_{i}^{*}-d_{i}}{d_{i}^{*}}\right \|$.  The square relative error $SqRel$ is defined as $SqRel=\frac{1}{N}\sum(\frac{d_{i}^{*}-d_{i}}{d_{i}^{*}})^{2}$. 
The root mean square error $rms$ is defined as 
$rms=\sqrt{\frac{1}{N}\sum {\left \|d_{i}^{*}-d_{i}\right \|}^{2}}$. 
The mean absolute logarithmic error $log_{10}$ is defined as 
$log_{10}=\frac{1}{N}\sum {\left \|log(d_{i}^{*})-log(d_{i})\right \|}$. These metrics are lower the better. The error metric describes the percentage of pixels with $\delta =max(\frac{d_{i}^{*}}{d_{i}},\frac{d_{i}}{d_{i}^{*}})<1.25^{k}(\delta_{1.25}^{k})$, $k$ = 1, 2 and 3 is also adopted to evaluate our performance, which are the higher the better. 

In all metrics $d_{i}^{*}$ is the ground truth depth value and $d_{i}$ denote the predict value at pixel $i$. Due to the scale ambiguities in monocular depth estimation, we follow Ranftl et al.~\cite{ranftl2019towards} to align the scale and shift using the least squares before computing errors. %\red{More details as well as a comparison of these benchmark datasets are summarized in Table~\ref{table:dataset}. }

\begin{figure*}
	\centering
	\includegraphics[width=0.99\linewidth]{widecomparison.pdf}\
	\vspace{-15pt}
	\caption{\red{Qualitative comparisons on unseen natural images from the Internet. Our method successfully boosts the performances of the backbone monocular depth estimation methods, and recovers the details in depth maps. SGR-GF and LeRes-GF denote the application of guided filter while SGR-Ours and LeRes-Ours denote the application of our method.}}
	\label{fig:widecomparison}
	%\vspace{-15pt}
\end{figure*}

% \begin{table}[t]
% 	\centering 
% 	\scalebox{0.7}{
% 		\begin{tabular}{c c c c c} 
% 			\hline 
% 			Datasets&$\#$scenes&Scene type&Metrics&Data type\\
% 			\hline
% 			Middlebury2021&24&Indoor&rel, rms, $\delta_{1.25}$&Structured-light\\
% 			\hline
% 			Multiscopic&100&Indoor&rel, rms, $\delta_{1.25}$&Synthetic\\
% 			\hline
% 		\end{tabular}
% 	}
% 	\caption{Details of benchmark datasets used in evaluations. }\label{table:dataset} 
% \end{table}

%we conduct several experiments to demonstrate the effectiveness of our method, including a comparison with state-of-the-art methods, a comparison of with or without our proposed guide mask, and a comparison of simplified network architecture. We also compared our method with the existing 融合？ method. 

\subsection{Comparisons to state-of-the-arts}\label{sec:comparison}

\noindent \textbf{Quantitative Evaluation} To evaluate the performances, we compare our method with some state-of-the-art monocular depth estimation alternatives in Table~\ref{table:quantitative}. Note that BMD~\cite{miangoleh2021boosting}, and 3DK~\cite{niklaus20193d} are two fusion based methods. To demonstrate that our self-supervised framework is effective, we also present the performance of monocular depth estimation methods applying with guided filter~\cite{he2010guided} directly. In the comparison, we adopt the trained models released by the authors and evaluate with their default configuration.

%When computing errors, we follow the processing pipeline of \cite{ranftl2019towards} and compare scale-invariant errors, since monocular depth estimation can only predict relative depth values. The performances on seven error metrics are shown in Table~\ref{table:quantitative}. While higher  $\delta_{1.25}$ is better, other metrics are the lower the better. 

\begin{figure*}
	\centering
	\includegraphics[width=0.99\linewidth]{zoomin.pdf}\
	\vspace{-15pt}
	\caption{Visual comparisons of our multi-resolution depth map fusion demonstrated on two backbone monocular depth estimation methods. Two local patches are zoomed in to show more details.  }
	\label{fig:zoomin}
	\vspace{-5pt}
\end{figure*}

Table~\ref{table:quantitative} demonstrate that our method can out perform all the other depth estimation alternative on most benchmarks and error metrics. Our method can also present better fusion results than guided filtering which is our training supervision. It means that our network takes advantages of both the low resolution input and the guided filtered fusion result but not strictly constrained by the self-supervision. The evaluation results demonstrate the superiority of our method over other state-of-the-art methods.

It should be noticed that our method was only pre-trained on LeRes. The trained fusion module can be easily migrated with other different monocular depth estimation networks like SGR with a short time of fine-tuning. Thus our method can be portable adopted with most state-of-the-art models. 
%We finally evaluate our multi-resolution depth fusion framework on two monocular depth estimation methods, SGR~\cite{xian2020structure} and  LeRes~\cite{yin2021learning}. We also compare the quality of our multi-resolution fusion network with several depth refinement methods including BMD~\cite{miangoleh2021boosting}, 3DK~\cite{niklaus20193d} and a baseline method guided filter~\cite{he2010guided}.

\noindent \textbf{Visual Comparison} The qualitative comparisons are presented in Figure~\ref{fig:widecomparison}. As discussed earlier, most monocular depth estimation methods suffer from blurry predictions. The improvement of detail-preserving by our multi-resolution depth map fusion is significant. Most details missing in the backbone methods are successfully recovered, while keeping the original depth values correct. Zoom-in examples are shown in Figure~\ref{fig:zoomin}, our fusion method can significantly improve performance of SGR~\cite{xian2020structure} and LeRes~\cite{yin2021learning}. %On different backbone methods, the proposed method successfully recovers details in depth maps. The quantitative evaluations are listed in Table~\ref{table:quantitative}. We adopt several error metrics, which are commonly used for depth estimation. 
%where the superiority of our multi-resolution depth fusion are more obvious. 
%fitting the scenario of the proposed multi-resolution framework. 

\noindent \textbf{Anti-noise Evaluation} The first advantage of our method over other fusion based methods like BMD is the noise robust enabled by our gradient-based fusion. Since BMD determine the fusion area explicitly by edge detection, its performance will drop significantly while the input include noise. We compare the anti-noise ability of our methods with BMD. We manually adopt Gauss noise to the input image, where the mean value of noise is 0 and the variance value changing from 0.001 to 0.009. Figure~\ref{fig:noise_line} shows the variety of $\delta_{1.25}$ value when adopting different variance of Gauss noise. Figure~\ref{fig:noise} present visualization examples of our method and BMD with or without Gauss noise. %We use LeRes as the backbone of BMD and ours, $*$ in Figure~\ref{fig:noise} denote the result with Gauss noise (variance is 0.006).

Fusion based methods like BMD can be easier influenced by the texture. We split the test benchmark into two sub-sets based on the edge number detected in the ground truth depth image, less edges denotes more difficult since it means more depth independent texture exist. The plot in Figure~\ref{fig:texture_vis} demonstrate our method can outperform BMD more on the difficult sub-set quantitatively. Figure~\ref{fig:texture_vis} also present a visual comparison on a difficult example, which BMD suffers from the texture noise.

\begin{figure}
	\centering
	\includegraphics[width=0.99\linewidth]{classvisual-plot.pdf}\
	\caption{Left: Quantitative evaluation between our method and BMD on a split benchmark. Ours outperform BMD more significant on the difficult subset. Right: Visual comparison between our method and BMD. From the left-top to right bottom: Input image, ground truth depth, depth estimation from low resolution input, BMD fusion result, depth estimation from high resolution input, Our result.}
	\label{fig:texture_vis}
\end{figure}

\noindent \textbf{Running time} Since our fusion module is one-step and requires no additional complex processing, our method is highly efficient. As introduced in Table~\ref{tab:ruuningtime}, our fusion module only takes 2\% processing time when comparing with LeRes for depth estimation of high resolution input. The whole pipeling of our method, which including the depth estimation time of low- and high resolution inputs, is still more than 16X faster than BMD.

\begin{figure}
	\centering
	\includegraphics[width=0.99\linewidth]{noise_line.pdf}\
	\caption{Quantitative evaluation of anti-noise ability of LeRes, BMD and ours. The vertical axis denote the value of $\delta_{1.25}$, which is the higher the better.}
	\label{fig:noise_line}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=0.99\linewidth]{noisecomp.pdf}\
	\caption{Comparisons of our method with a state-of-the-art depth fusion method~\cite{miangoleh2021boosting} on the same backbone single-resolution depth estimation method LeRes~\cite{yin2021learning} on images with Gaussian noises. $*$ denote the result from image with higher Gauss noise.It shows that our method is more robust to image noises, where BMD~\cite{miangoleh2021boosting} introduces more artifacts.  }
	\label{fig:noise}
\end{figure}



%Through the whole evaluation, we adopt LeRes~\cite{yin2021learning} as the backbone method of BMD. For guided filter parameters radius and regularization, we fixed at $\frac{W_{i}}{12}$ and $10^{-12}$ (${W_{i}}$ denote the width of the input image). And for the input resolution, we adopt $W_{b}$ (original size) for backbone to predict low-res depth while using $W_{b} * \frac{r}{2}$ to predict high-res depth ($r$ is the upscale parameter, through the experiments we fixed $r$ at 3). 

\begin{table}[t]
\scalebox{0.825}{
\centering
\begin{tabular}{l|l|l|l}
\hline
Method & Task & Time per frame & GFLOPS \\ 
\hline
\multirow{2}{*}{LeRes} & pred low-res depth & 0.0240s & 95.88092G \\ 
\cline{2-4}
 & pred high-res depth & 0.0958s & 862.92825G \\ 
\hline
\multirow{2}{*}{SGR} & pred low-res depth & 0.0282s & 95.88092G \\ 
\cline{2-4}
 & pred high-res depth & 0.0981s & 862.92825G \\ 
\hline
3DK & pred refinement depth & 0.0141s & 118.02850G \\ 
\hline
BMD & pred refinement depth & 14.614s & 14834.4784G \\ 
\hline
Guided Filter & fuse low-res and high-res & 0.7025s & - \\ 
\hline
Ours & fuse low-res and high-res & 0.0653s & 17.68863G\\\hline
\end{tabular}}
\caption{Running time statistics.}\label{tab:ruuningtime}
\vspace{-15pt}
\end{table}


\subsection{Ablation studies}\label{sec:ablations}

We evaluate the influence of following designs during training. For fair comparisons, all ablation alternatives are both trained for 30 epochs, and training configurations are set as the same. %Our full performance after 150 epochs are in Table~\ref{table:quantitative}. 
%We adopt guided filter to get a enhanced fused depth, where the radius and regularization are fixed at $\frac{W_{i}}{12}$ and $1e-12$ (${W_{i}}$ (${W_{i}}$ denote the width of the input image).

We first investigated the effects on model performance of different type of loss function, including ILNR loss, gradient loss\cite{li2018megadepth} and ranking loss. We construct the ablation study with 7 different setting of training loss as shown in Table~\ref{table:ablation}. We adopt ILNR loss to supervise the value domain in our fusion network with low resolution result and guided fused result, and adopt gradient loss\cite{li2018megadepth}, original ranking loss\cite{xian2020structure} and the proposed ranking loss to supervise the gradient domain with high resolution result and guided fused result. 
%In setting A, we use gradient loss\cite{} to learn the gradient from high-res backbone result while utilize ILNR loss to keep the value of low-res backbone result. As a contrast, we use guided filter to get a guided depth and learn the gradient and depth value from guided depth instead in setting D. In setting B, we use ILNR loss to learn the value of low-res depth while utilize the original ranking loss\cite{xian2020structure} to learn the detail from high-res depth. In setting F(our final design), we train the network with ILNR loss and our ranking loss, optimize the difference between fusion result and guided depth.
Table~\ref{table:ablation} shows that our configuration outperform other alternatives. The visual example presented in supplementary also demonstrate that the proposed loss function and optimization target can lead to a better performance for recovering the detail.

We also evaluate the validation of our differential gradient-domain composition design. We compare the depth estimation performance with and without $\mathcal{E}_g$. The result in Table~\ref{tab:e_g_ablation} demonstrate that this simple design is critical and can significantly improve the detail preserving performance. The visual comparison is presented in Figure~\ref{fig:vis_g_layer} and more can be found in the supplementary.


%Optimization target:

%In order to illustrate the effectiveness of our designed optimization target, the four settings can be seen as two comparison groups - Setting A with Setting C, Setting B with Setting D. Two comparison groups have the same adoption of loss function respectively, and the setting utilize guided depth has the lower error in each group. 


%Loss type:

%Similarly, the four settings can be seen as two comparison groups - Setting A with Setting B, Setting C with Setting D, to demonstrate the effectiveness of our ranking loss.  The settings in each group use ILNR loss to preserve the depth, while using ranking loss improve the ability of recovering the detail. Quantitative result and qualitative result improvements can be easily find in Fig~\ref{fig:loss} and  Tab~\ref{table:ablation}



\begin{table}
\centering
\scalebox{0.9}{
\begin{tabular}{c|ccccccc} 
\hline
Method & AbsRel\downarrow & SqRel\downarrow & rms\downarrow & log10\downarrow & \delta_{1}\uparrow & \delta_{2}\uparrow & \delta_{3}\uparrow \\ 
\hline
w/ & 0.143 & 0.021 & 0.087 & 0.057 & 0.835 & 0.953 & 0.983 \\ 
\hline
w/o & 0.156 & 0.023 & 0.095 & 0.062 & 0.811 & 0.946 & 0.981 \\
\hline
\end{tabular}}
\caption{Comparison of our architecture with and without the first convolution layer of high-resolution depth.}\label{tab:e_g_ablation}
\end{table}


%\red{To demonstrate the effectiveness of the 3-layer fusion network, we train a 2-layer version. We adopt LeRes~\cite{yin2021learning} with resNeXt101\cite{xie2017aggregated} as the backbone single-resolution depth prediction method and compare the 2-layer network with the 3-layer network on iBims-1\cite{koch2018evaluation}. The errors are shown in Table~\ref{table:ablation}. We evaluate the absolute mean relative error ($AbsRel$),  root mean square error($rms$) and the boundary metrics $\varepsilon _{DBE}^{acc}$ and $\varepsilon _{DBE}^{comp}$ from \cite{koch2018evaluation}. It shows that the 2-layer version is too simple to complete the fusion well, and compare to the backbone single-resolution method LeRes, the improvement by 2-layer fusion is minor. The 3-layer version in the proposed method boosts the performance under various metrics. }

% \begin{figure}
% 	\centering
% 	\includegraphics[width=0.99\linewidth]{loss.pdf}\
% 	\caption{\red{Visual comparisons of different loss function settings. Our proposed ranking loss can effectively improve the detail(B and D).}}
% 	\label{fig:loss}
% \end{figure}


% \begin{figure}
% 	\centering
% 	\includegraphics[width=0.99\linewidth]{classcompare.pdf}\
% 	\caption{.}
% 	\label{fig:texture_plot}
% \end{figure}

\subsection{Limitations}

%Since our method is based on any backbone monocular depth estimation and improves their results with much more details. A problem is when the backbone method generates inaccurate depth predictions, in order words, when the three-resolution depth maps are all implausible in depth values. Our method cannot fix the inaccurate depth values and still get a plausible fusion results. 
Our method fuses details recovered from depth predictions of high-resolution images into predictions of low-resolution images, to improve the performance of the backbone method. However if the original resolution of input images are low, the improvements by our multi-resolution depth fusion are minor. Moreover, with recent successes of introducing scene analysis into 3D vision tasks, our method may be better incorporating with scene analysis such as edges, boundaries or plane detection. Introducing semantics into this task is also a promising future direction. 
%Semantic information that can be predicted to better supervise or constrain the monocular depth estimation problem. 
%Incorporating this problem with another highly-related problem, image segmentation, is also worthy to explore. Both tasks can be very helpful to each other, and a joint training may lead to boosts of both tasks. 
% \begin{table}[t]
% \centering
% \scalebox{0.7}{
% \begin{tabular}{c|ccc|c} 
% \hline
% \multirow{2}{*}{} & \multicolumn{3}{c|}{Loss function} & Result \\ 
% \cline{2-5}
%  & ILNR & Gradient & Ranking & error \\ 
% \hline
% Setting A & Low-res depth & High-res depth & x & 0.734 \\
% Setting B & Low-res depth & \cross & High-res depth & \uline{0.688} \\
% Setting C & Guided depth & Guided depth & x & 0.723 \\
% \hline
% Setting D & Guided depth & x & Guided depth & \textbf{0.684} \\
% \hline

% \end{tabular}}

% \label{table:ablation} 
% \end{table}

\begin{table}[t]
\centering
\scalebox{0.7}{
\arrayrulecolor{black}
\begin{tabular}{c|cccc|c} 
\hline
\multirow{2}{*}{} & \multicolumn{4}{c|}{Loss function} & Result \\ 
\cline{2-6}
 & ILNR & Gradient & SGR Ranking & Ours Ranking & error \\ 
\cline{1-5}\arrayrulecolor{black}\cline{6-6}
Setting A & Low-res depth & High-res depth & \times & \times & 0.734 \\
Setting B & Low-res depth & \times & High-res depth & \times & 0.722 \\
Setting C & Low-res depth & \times & \times & High-res depth & \uline{0.688} \\
Setting D & Guided depth & Guided depth & \times & \times & 0.723 \\
Setting E & Guided depth & \times & Guided depth & \times & 0.714 \\
Setting F & Guided depth & \times & \times & Guided depth & 0.711 \\
\arrayrulecolor{black}\hline
Ours & Low-res depth & \times & \times & Guided depth & \textbf{0.684} \\
\hline
\end{tabular}}
\caption{Ablation study with different training settings. Here setting F is our final setting and error calculation we follow Xian et al.\cite{xian2020structure}}
\label{table:ablation} 
\vspace{-5pt}
\end{table}

